Evidential Softmax for Sparse Multimodal Distributions in Deep Generative Models

Many applications of generative models rely on the marginalization of their high-dimensional output probability distributions. Normalization functions that yield sparse probability distributions can make exact marginalization more computationally tractable. However, sparse normalization functions usually require alternative loss functions for training since the log-likelihood is undefined for sparse probability distributions. Furthermore, many sparse normalization functions often collapse the multimodality of distributions. In this work, we present $\textit{ev-softmax}$, a sparse normalization function that preserves the multimodality of probability distributions. We derive its properties, including its gradient in closed-form, and introduce a continuous family of approximations to $\textit{ev-softmax}$ that have full support and can be trained with probabilistic loss functions such as negative log-likelihood and Kullback-Leibler divergence. We evaluate our method on a variety of generative models, including variational autoencoders and auto-regressive architectures. Our method outperforms existing dense and sparse normalization techniques in distributional accuracy. We demonstrate that $\textit{ev-softmax}$ successfully reduces the dimensionality of probability distributions while maintaining multimodality.

==> Archives/05-discussion.tex <==
\section{Results and Discussion}
In this work, we propose the evidential softmax transformation and its training form to allow for training conditional variational autoencoders with sparse multimodal latent spaces. We show the connection between this transformation and the post-hoc sparsification method using evidential theory introduced in \cite{itkina_evidential_2021} and provide theoretical properties of the transformation. We provide a modification to the function during training time to allow logarithms of the output distributions to remain defined and show its similarity in properties to the softmax function. We show that this approach compares favorably to state-of-the-art methods in semi-supervised learning and conditional models.

% Future work includes identifying and implementing more experiments which show the advantages and disadvantages of this method. In addition, there is potential for further theoretical investigation: in particular, there could be a Bayesian interpretation of this method, with some prior which encourages sparsity; or this could be a sort of constrained optimization in a similar way to the lasso regression as a constrained optimization on the $\ell_1$ norm of weights.

==> Archives/exploration.tex <==
\section{Finding a closed-form solution} 
\medskip 

Given a $J$-dimensional feature vector $\phi \in \R^J$ (with $\phi_0 = 1$ as the bias term for notational simplicity), we constuct the post-hoc evidentially sparsifying softmax function $f: \R^J \to \Delta^K$ that maps to a probability function in the $K$-dimensional simplex. \\ \\
The function $f$ is parameterized by $\beta \in \R^{K \times J}$. Define $w = \beta \phi \in \R^K$. Note that we actually don't really care about the $j$ index in the individual evidential weights $w_{jk}$ in the paper since $w_{1k} = w_{2k} = \ldots = w_{Jk}$. Then we write $w^+ = \max(0, w)$ and $w^- = \max(0, -w)$, where the $\max$ operation is applied to each index of the vector (aside: this is exactly ReLU). \\ \\
We first express $w$ in terms of the neural network weights $\hat{\beta}$. Using the notational simplification of index 1 being the bias term, equations (7) and (8) in the evidential sparsification paper give
\begin{align*}
    w_{jk} &= \frac{1}{J} \sum_{j = 1}^J \beta_{jk} \phi_j \\
    \beta_{jk} &= \hat{\beta}_{jk} - \frac{1}{K} \sum_{\ell = 1}^K \hat{\beta}_{j \ell}
\end{align*}
Let $\overline{\beta}_{j} = \frac{1}{K}\sum_{\ell=1}^K \hat{\beta}_{j\ell}$. Then plugging in the second equation into the first and summing over $j$ gives
$$w_k = \sum_{j = 1}^J \beta_{jk} \phi_j = \sum_{j=1}^J \left(\hat{\beta}_{jk} - \overline{\beta}_j\right) \phi_j$$
or in matrix notation $w = \hat{\beta} \phi - \overline{\beta} \phi$. This gives the weights in terms of the input feature vector $\phi$ and the weights learned by the neural network $w$. \\ \\
Next, we derive the sparsification relation in terms of $w$. The mass function is some scary-looking thing like
$$m(\{z_k\}) = Ce^{-w_k^-} \left(e^{w_k^+} - 1 + \prod_{\ell \ne k}\left(1 - e^{-w_\ell^-}\right)\right)$$
but luckily what we really care about is $\I\{m(\{z_k\}) \ne 0\}$, which happens if one of the following is true:

\begin{enumerate}
    \item $w_k^+ \ne 0$, or
    \item $w_\ell^- \ne 0$ for all $\ell \ne k$
\end{enumerate}
We can rewrite these as two equivalent conditions:
\begin{align}
    1. \; w_k &> 0 \label{cond_1} \\
    2. \; w_\ell &<0 \; \forall\ell \ne k\label{cond_2}  
\end{align}
Intuitively, if we only had the first condition, then the post-hoc solution would be equivalent to $\Relu$ on the softmax output, followed by rescaling. The second condition is essentially a relaxation on the $\Relu$ when no other class has a strong weight. \\ \\
The asymmetry in Equation \ref{cond_2} is a bit annoying, so I think it would be nice to make one very slight relaxation to the conditions to give
\begin{equation}
    w_\ell <0 \; \forall \ell \in [K] \label{cond_2_relaxed}
\end{equation}
The difference between the Equations \ref{cond_2} and \ref{cond_2_relaxed} occurs when $w_k \ge 0$ but $w_\ell < 0$ for all $\ell \ne k$. But note that if we have strict equality, where $w_k > 0$, then Equation \ref{cond_1} is actually true and the final results are equivalent. Therefore, the only instance where the conditions give different results is if $w_k = 0$ and $w_\ell < 0$ for all $\ell \ne k$, and since $w$ is in continuous space, this occurs with probability $0$. \\ \\
\section{Questions}
\subsection{Question 1: Does this really imply that sparsification happens completely based off of the weights $w = \beta \phi$?}

To me, this seems a bit surprising. We started with evidential theory, but the condition for the mass function being nonzero has nothing to do with D-S theory anymore since Appendix B of the Evidential Sparsification paper proves that the $\alpha_{jk}, \beta_{jk}$ coefficients result in weights that are equivalent to those of softmax. \\ \\
This means that the weights $w = \beta \phi$ are exactly the same as ones with normal softmax, which implies that equations \ref{cond_1} and \ref{cond_2} in principle have can be completely decoupled with D-S theory. Is the above all correct, and if so, do we have a sparsification method operates solely on $w$? \\ \\
If so, then this is essentially exactly like the setup of sparsemax, since we don't really care about the $\alpha_{jk}, \beta_{jk}$ parameters - all that matters is an input $w \in \R^K$, the indicator function that performs sparsification, and the output probability weights $p$.


==> Sections/checklist.tex <==
\section*{Checklist}
\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{See \cref{section:evidential_softmax,section:experiments}}
  \item Did you describe the limitations of your work?
    \answerYes{See \cref{section:broader_impact}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See \cref{section:broader_impact}}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{See \cref{section:evidential_softmax}}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{They are attached in supplemental materials.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See supplemental materials.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See supplemental materials.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{See \cref{section:experiments}}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See \cref{section:experiments}}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerNA{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}



==> includes.tex <==
\usepackage{amsmath,amssymb,amsfonts,amsthm,epsfig, bbm}
%\usepackage[usenames,dvipsnames]{xcolor}

%\usepackage{bm,xspace}

%\usepackage{cancel}
%\usepackage{fullpage}
%\usepackage{framed}
% \usepackage{verbatim}
%\usepackage{enumitem}
%\usepackage{multirow}
%\usepackage{afterpage}
%\usepackage{mathrsfs}  
%\usepackage{algorithm2e}

%\usepackage[normalem]{ulem}
\usepackage{caption} 
%\usepackage[english]{babel}
%\usepackage{amsmath}
%\usepackage{bbm}
\usepackage{xcolor}
\usepackage[style=ieee,natbib=true,url=false,doi=false,mincitenames=1]{biblatex}
\AtBeginBibliography{\small}
% \addbibresource{refs.bib}
